KROMA: Ontology Matching with Knowledge Retrieval and Large Language Models

Ontology Matching (OM) is a cornerstone task of semantic interoperability, yet existing systems often rely on handcrafted rules or specialized models with limited adaptability. We present KROMA, a novel OM framework that harnesses Large Language Models (LLMs) within a Retrieval-Augmented Generation (RAG) pipeline to dynamically enrich the semantic context of OM tasks with structural, lexical, and definitional knowledge. To optimize both performance and efficiency, KROMA integrates a bisimilarity-based concept matching and a lightweight ontology refinement step, which prune candidate concepts and substantially reduce the communication overhead from invoking LLMs. Through experiments on multiple benchmark datasets, we show that integrating knowledge retrieval with context-augmented LLMs significantly enhances ontology matching, outperforming both classic OM systems and cutting-edge LLM-based approaches while keeping communication overhead comparable. Our study highlights the feasibility and benefit of the proposed optimization techniques (targeted knowledge retrieval, prompt enrichment, and ontology refinement) for ontology matching at scale.

==> assets/algo1_bisimmatch.tex <==
\begin{algorithm}[ht]
\caption{Offline Refinement}\label{alg:offline_refined}
\begin{algorithmic}[1]
  \State \textbf{Input:} source ontology \(O_S=(C_S,E_S)\), target ontology \(O_T=(C_T,E_T)\), initial alignment \(A\subseteq C_S\times C_T\)
  \State \textbf{Output:} refined alignment \(A'\)
  \State \(V\gets C_S\cup C_T,\quad E\gets E_S\cup E_T\cup A,\quad G\gets(V,E)\)
  \State compute \(r(c)\) for all \(c\in V\)
  \State \(\rho\gets\max_{c\in V}r(c)\), and for each \(i=0,\dots,\rho\) let  
    \(\;B_i=\{\,c\in V : r(c)=i\}\)
  \State \(\mathcal{P}\gets\{B_0,\dots,B_\rho\}\)
  \State \textbf{for} \(i=0,\dots,\rho\) \textbf{do}
    \begin{compactitem}
      \item collapse each block \(X\in\mathcal{P}\) with \(X\subseteq B_i\)
      \item for each \(c\in B_i\) and each block \(C\in\mathcal{P}\) with \(C\subseteq\bigcup_{j>i}B_j\):
        \[
          C_1=\{\,x\in C : (x,c)\in E\},\quad
          C_2=C\setminus C_1,
          \quad\mathcal{P}\gets(\mathcal{P}\setminus\{C\})\cup\{C_1,C_2\}
        \]
    \end{compactitem}
  \State \(A'\gets\{(s,t)\in C_S\times C_T : \exists\,B\in\mathcal{P}\text{ with }\{s,t\}\subseteq B\}\)
\end{algorithmic}
\end{algorithm}

==> assets/algo2_ontorefine.tex <==
\begin{algorithm}[ht]
\caption{Ontology Refinement}\label{alg:refine}
\begin{algorithmic}[1]
  \REQUIRE Ontologies $O_S,O_T$, current compressed graph $\mathcal{G}_r$, update batch $\Delta\mathcal{G}$
  \ENSURE Updated compressed graph $\mathcal{G}_r\oplus\Delta\mathcal{G}_r$
  \STATE initialize $\mathsf{ExpertQueries}\gets\emptyset$
  \STATE recompute $\mathit{rank}(\cdot)$ in $\mathcal{G}_r$ w.r.t.\ $\Delta\mathcal{G}$
  \STATE apply those rank updates to $\mathcal{G}_r$
  \FORALL{insertion $e=(u\to u')\in \Delta\mathcal{G}$ in ascending $\mathit{rank}(u)$}
    \STATE $(\mathcal{G}_r,\mathsf{newQ})
           \gets \mathsf{incRCM}^+(e,\,[u]_{R_e},\,[u']_{R_e},\,\mathcal{G}_r)$
    \STATE $\mathsf{ExpertQueries}\gets \mathsf{ExpertQueries}\cup\mathsf{newQ}$
  \ENDFOR
  \FORALL{$(x,y)\in \mathsf{ExpertQueries}$}
    \STATE query human expert on $(x,y)$ and merge if confirmed
  \ENDFOR
  \RETURN $\mathcal{G}_r$
\end{algorithmic}
\end{algorithm}

\begin{algorithm}[ht]
\caption{Procedure \(\mathsf{incRCM}^+\)}\label{alg:incrcm}
\begin{algorithmic}[1]
  \REQUIRE Compressed graph $\mathcal{G}_r=(V_r,E_r)$, insertion $e=(u\!\to\!u')$, super‐nodes $[u]_{R_e},[u']_{R_e}$
  \ENSURE Updated $\mathcal{G}_r$ and expert queries $\mathsf{newQ}$
  \STATE initialize $\mathsf{newQ}\gets\emptyset$
  \STATE $\mathsf{Split}(u,u',[u]_{R_e},[u']_{R_e})$
  \IF{$\mathit{rank}([u]_{R_e})>\mathit{rank}([u']_{R_e})$}
    \FORALL{$v\in \mathcal{B}([u]_{R_e})$}
      \STATE $\mathsf{Merge}(\{u\},v)$
    \ENDFOR
    \FORALL{$v'\in \mathcal{B}([u']_{R_e})$}
      \STATE $\mathsf{Merge}(\{u'\},v')$
    \ENDFOR
  \ELSIF{$\mathit{rank}([u]_{R_e})=\mathit{rank}([u']_{R_e})$}
    \FORALL{$v\in \mathcal{P}([u']_{R_e})$}
      \STATE $\mathsf{Merge}(\{u\},v)$
    \ENDFOR
    \FORALL{$v'\in \mathcal{C}([u]_{R_e})$}
      \STATE $\mathsf{Merge}(\{u'\},v')$
    \ENDFOR
  \ELSE
    \STATE $\mathsf{newQ}\gets \mathsf{newQ}\cup\{(u,u')\}$
     \Comment{inconsistent ranks $\rightarrow$ expert needed}
  \ENDIF
  \RETURN $\mathcal{G}_r,\;\mathsf{newQ}$
\end{algorithmic}
\end{algorithm}

==> assets/figures.tex <==
% \begin{figure}[!htbp]
%     \centering
%     \includegraphics[width=\textwidth]{iswc2025/figs/performance_models.png}
%     \caption{Performance}
%     \label{fig:perf}
% \end{figure}

% -------- KROMA MODELS --------
% \begin{figure}[!htbp]
%     \centering
%     \caption{Models}
%     \label{fig:kroma_models}
% \end{figure}
% ----------------

% -------- SCALE --------
% \begin{figure}[!htbp]
%     \centering    \includegraphics[width=\textwidth]{iswc2025/figs/scale.png}
%     \caption{Scalability}
%     \label{fig:scale}
% \end{figure}
% ----------------

% % -------- LONG SHORT TOKEN USAGE --------
% \begin{figure}[!htbp]
%     \centering
%     \includegraphics[width=\textwidth]{iswc2025/figs/longshort_token_usage.pdf}
%     \caption{Token Usage of Short and Long Reasoning LLMs on Anatomy's Mouse–Human Dataset}
%     \label{fig:longshort_token_usage}
% \end{figure}
% % ----------------------------

% -------- API CALL REDUCTION --------
% \begin{figure}[!htbp]
%     \centering
%     \caption{API Call by Dataset and Model}
%     \label{fig:api_reduce}
% \end{figure}
% ----------------------------

% -------- LONG SHORT PERFORMANCE --------
% \begin{figure}[!htbp]
%     \centering
%     \includegraphics[width=\textwidth]{iswc2025/figs/longshort_perf.png}
%     \caption{Short vs. Long Reasoning LLM Performance}
%     \label{fig:longshort_perf}
% \end{figure}
% ----------------------------

% % -------- TOKEN USAGE --------
% \begin{figure}[!htbp]
%     \centering
%     % Scale to 0.7 of text width
%     \includegraphics[width=\textwidth]{iswc2025/figs/token_usage.pdf}
%     \caption{Token usage comparison across three LLMs on four ontology‑matching tasks (Mouse–Human, Nell–DBpedia, ENVO–SWEET, MI–MatOnto), showing total input tokens (top row), total output tokens (middle row), and average tokens per API call (bottom row).}
%     \label{fig:token_usage}
% \end{figure}
% % ----------------------------

% % -------- GPT CONFIDENCE --------
% \begin{figure}[!htbp]
%     \centering
%     \includegraphics[width=\textwidth]{iswc2025/figs/confidence/gpt-4o-mini_confidence_grid.png}
%     \caption{Confidence versus correctness for GPT-4o-mini on six ontology‑matching tasks. The heatmap shows prediction counts by confidence bin (x‑axis), split into correct (top row) and incorrect (bottom row). GPT‑4o‑mini concentrates most correct matches at the highest confidence levels (9–11) with minimal errors, indicating strong calibration.}
%     \label{fig:gpt_confidence}
% \end{figure}
% % ----------------------------

% % -------- LLAMA-3.3 CONFIDENCE --------
% \begin{figure}[!htbp]
%     \centering
%     \includegraphics[width=\textwidth]{iswc2025/figs/confidence/meta-llama_Llama-3.3-70B-Instruct-Turbo-Free_confidence_grid.png}
%     \caption{Confidence versus correctness for Llama‑3.3‑70B across six ontology‑matching tasks. Each heatmap cell indicates the count of predictions in each confidence bin (x‑axis), separated into correct (top row) and wrong (bottom row). Llama‑3.3‑70B clusters most correct answers in the highest bins (9–11) but shows occasional errors even at top confidence, suggesting slight overconfidence.}
%     \label{fig:llama_confidence}
% \end{figure}
% % ----------------------------

% % -------- QWEN-1.5B CONFIDENCE --------
% \begin{figure}[!htbp]
%     \centering
%     \includegraphics[width=\textwidth]{iswc2025/figs/confidence/deepseek-ai_DeepSeek-R1-Distill-Qwen-1.5B_confidence_grid.png}
%     \caption{Confidence versus correctness for Qwen‑1.5B on six ontology‑matching tasks. Each grid cell shows the number of predictions at a given confidence bin (x‑axis) split by correct (top row) and wrong (bottom row). Qwen‑1.5B’s errors concentrate in mid‑range confidence (7–9), while its highest bin (10–11) is almost exclusively correct, indicating strong calibration.}
%     \label{fig:qwen_confidence}
% \end{figure}
% % ----------------------------

==> assets/misc.tex <==
% \begin{table}[!htb]
%   \centering
% \end{table}

\begin{table}[!htb]
  \centering
  %% (b) KROMA zero-shot performance
  \begin{subtable}[t]{\linewidth}
    \centering
    \setlength{\tabcolsep}{3pt}
    \resizebox{\textwidth}{!}{%
      \begin{tabular}{ll *{3}{ccc} |ccc}
        \toprule
        \multicolumn{2}{c}{\bfseries Task / Model} &
          \multicolumn{3}{c}{\bfseries Qwen2.5-1.5B} &
          \multicolumn{3}{c}{\bfseries GPT-4o-mini} &
          \multicolumn{3}{c}{\bfseries Llama-3.3-70B} &
          \multicolumn{3}{c}{\bfseries OM-LLM} \\
        \cmidrule(lr){1-2} \cmidrule(lr){3-5}
        \cmidrule(lr){6-8} \cmidrule(lr){9-11}
        \cmidrule(lr){12-14}
        {\bfseries Task} & & $P$ & $R$ & $F_1$ & $P$ & $R$ & $F_1$ & $P$ & $R$ & $F_1$ & $P$ & $R$ & $F_1$ \\
        \midrule
        Mouse-Human   & & 84.66 & 82.52 & 83.58 & 85.12 & 100.00 & 91.96 & 90.78  & 99.50 & \textbf{94.94} & 97.40 & 87.50 & 92.20 \\
        NCIT-DOID     & & 95.00 & 100.00 & \bfseries97.44 & 95.24 & 100.00 & \bfseries97.56 & 97.59 & 99.69 & \bfseries98.63 & 96.40 & 93.20 & 94.80 \\
        Nell-DBpedia  & & 96.30 & 94.10  & 95.02          & 95.89 & 95.64  & 95.67          & 94.32 & 100.00 & \textbf{97.08} & 100.00 & 92.20 & 96.00 \\
        YAGO-Wikidata & & 93.81 & 97.15  & \bfseries95.45  & 93.79 & 97.14  & \bfseries95.44  & 91.80 & 99.60  & \bfseries95.54  & 100.00 & 85.52 & 92.19 \\
        ENVO-SWEET    & & 87.37 & 73.45  & 79.80          & 87.23 & 100.00 & \textbf{93.18} & 87.16 & 97.29  & \textbf{91.95} & 80.30 & 59.50 & 83.70 \\
        MI-MatOnto    & & 45.74 & 92.69  & \bfseries61.25  & 46.08 & 89.70  & \bfseries60.88  & 46.68 & 93.36  & \bfseries62.24  & 89.70 & 20.19 & 32.97 \\
        \bottomrule
      \end{tabular}
    }
    \subcaption{Performance across six tasks using three LLMs. Bold $F_1$ indicates where KROMA beats the best existing OM-LLM.}
    \label{tab:sub:b_kroma}
  \end{subtable}
  \begin{subtable}[t]{\linewidth}
    \centering
    \begin{tabular}{llll}
      \toprule
      \textbf{Code} & \textbf{System} & \textbf{Variant} & \textbf{Version} \\ \midrule
      KL3.3    & KROMA  & –  & Llama-3.3-70B   \\
      KNR3.3   & KROMA  & NR & Llama-3.3-70B   \\
      KNB3.3   & KROMA  & NB & Llama-3.3-70B   \\
      KNB3.2   & KROMA  & NB & Llama-3.2-3B   \\
      KL3.1    & KROMA  & –  & Llama-3.1-70B   \\
      KL2.0    & KROMA  & –  & Llama-2-70B     \\
      K4mini    & KROMA  & –  & GPT-4o-mini   \\
      KNR4mini   & KROMA  & NR & GPT-4o-mini   \\
      KNB4mini   & KROMA  & NB & GPT-4o-mini   \\
      KG2    & KROMA  & –  & Gemma-2B     \\
      KM7    & KROMA  & –  & Mistral-7B     \\
      ML3.1    & MILA   & –  & Llama-3.1-70B   \\
      OL2.0    & OLaLa  & –  & Llama-2-70B     \\
      L4G3.5   & LLM4OM & –  & GPT-3.5-175B    \\
      L4L2   & LLM4OM & –  & Llama-2-7B    \\
      L4MPT   & LLM4OM & –  & MPT-7B    \\ 
      LLFT   & LLM4OM & –  & Flan-T5-XXL    \\ 
      \bottomrule
    \end{tabular}
    \subcaption{Abbreviation mapping for model codes.}
    \label{tab:sub:codes}
  \end{subtable}
\end{table}

\begin{table}[!htb]
  \centering
  %% (a) MMLU benchmark
  \begin{subtable}[t]{\linewidth}
    \centering
    \begin{tabular}{lcc}
      \toprule
      \textbf{Model}   & \textbf{Parameters} & \textbf{MMLU Score (\%)} \\
      \midrule
      Gemma-2B         & 2B                  & 51.3                     \\
      Flan-T5-XXL      & 11B                 & 55.1                     \\
      Llama-3.2-3B     & 3B                  & 63.4                     \\
      Llama-2-7B       & 7B                  & 68.9                     \\
      Mistral-7B       & 7B                  & 60.1                     \\
      \bottomrule
    \end{tabular}
    \subcaption{Benchmark comparison of models based on MMLU (5-shot, top-1).}
    \label{tab:sub:a_mmlu}
  \end{subtable}
  %% (h) KROMA vs. Others
  % \begin{subtable}[t]{\linewidth}
  %   \centering
  %   \small
  %   \resizebox{\textwidth}{!}{%
  %     \begin{tabular}{|l|l|c|c|c|}
  %       \hline
  %       {\bfseries Dataset} & {\bfseries Model}              & {\bfseries P} & {\bfseries R} & {\bfseries $F_1$} \\ \hline
  %       \multirow{8}{*}{Mouse-Human}
  %         & KROMA + Llama-3.3-70B     & 90.78 & 99.50 & \textbf{94.94} \\
  %         & KROMA-NR + Llama-3.3-70B & 92.34 & 90.16 & 91.25        \\
  %         & KROMA-NB + Llama-3.3-70B &100.00 & 76.36 & 86.59        \\
  %         & KROMA + Llama-3.1-70B    & 90.42 & 99.00 & 94.50        \\
  %         & KROMA + Llama-2-70B      &100.00 & 87.34 & 93.24        \\
  %         & MILA + Llama-3.1-70B     &100.00 & 87.50 & 92.20        \\
  %         & OLaLa + Llama-2-70B      & 91.40 & 89.10 & 90.20        \\  
  %         & LLM4OM + GPT-3.5-175B    & 90.82 & 87.46 & 89.11        \\ \hline
  %       \multirow{8}{*}{NCIT-DOID}
  %         & KROMA + Llama-3.3-70B     & 97.59 & 99.69 & \textbf{98.63} \\
  %         & KROMA-NR + Llama-3.3-70B & 93.20 & 96.90 & 95.01        \\
  %         & KROMA-NB + Llama-3.3-70B & 83.33 &100.00 & 90.91        \\
  %         & KROMA + Llama-3.1-70B    & 97.43 & 99.08 & 98.24        \\
  %         & KROMA + Gemma-2B         & 66.67 &100.00 & 80.00        \\
  %         & MILA + Llama-3.1-70B     & 96.40 & 93.20 & 94.80        \\
  %         & LLMap + Flan-T5-XXL      & 86.10 & 62.00 & 72.10        \\
  %         & LLM4OM + GPT-3.5-175B    & 86.19 & 80.06 & 83.01        \\ \hline
  %       \multirow{6}{*}{Nell-DBpedia}
  %         & KROMA + Llama-3.3-70B     & 94.32 &100.00 & \textbf{97.08} \\
  %         & KROMA-NR + Llama-3.3-70B & 97.46 & 91.27 & 94.26        \\
  %         & KROMA-NB + Llama-3.3-70B & 91.17 & 96.12 & 93.58        \\
  %         & KROMA + Llama-2-70B      & 95.50 & 96.55 & 96.02        \\
  %         & OLaLa + Llama-2-70B      &100.00 & 92.20 & 96.00        \\
  %         & LLM4OM + GPT-3.5-175B    &100.00 & 89.14 & 94.26        \\ \hline
  %       \multirow{5}{*}{YAGO-Wikidata}
  %         & KROMA + Llama-3.3-70B      & 91.80 & 99.60 & 95.54 \\
  %         & KROMA-NR + Llama-3.3-70B   & 93.50 & 90.50 & 91.98 \\
  %         & KROMA-NB + Llama-3.3-70B   & 90.50 & 89.00 & 89.74 \\
  %         & KROMA + Llama-3.2-3B       & 89.09 & 98.00 & 93.33 \\
  %         & LLM4OM + Llama-2-7B        &100.00 & 85.52 & 92.19 \\ \hline
  %       \multirow{9}{*}{ENVO-SWEET}
  %         & KROMA + GPT-4o-mini        & 87.23 &100.00 & \textbf{93.18} \\
  %         & KROMA-NR + GPT-4o-mini     & 86.90 & 98.00 & 92.12        \\
  %         & KROMA-NB + GPT-4o-mini     & 82.00 & 88.00 & 84.89        \\
  %         & KROMA + Llama-3.1-70B      & 87.11 & 96.19 & 91.43        \\
  %         & KROMA + Llama-2-70B        & 92.50 & 78.72 & 85.06        \\
  %         & KROMA + Mistral-7B         & 87.19 & 99.59 & 92.98        \\
  %         & MILA + Llama-3.1-70B       & 80.30 & 59.50 & 83.70        \\
  %         & OLaLa + Llama-2-70B        & 43.10 & 61.30 & 51.10        \\
  %         & LLM4OM + Mistral-7B        & 59.00 & 51.67 & 55.09        \\ \hline
  %       \multirow{5}{*}{MI-MatOnto}
  %         & KROMA + Llama-3.3-70B      & 45.74 & 92.69 & \textbf{61.25} \\
  %         & KROMA-NR + Llama-3.3-70B   & 44.80 & 91.40 & 59.95        \\
  %         & KROMA-NB + Llama-3.3-70B   & 42.00 & 85.00 & 55.00        \\
  %         & KROMA + Llama-3.2-3B       & 56.36 & 62.00 & 59.05        \\
  %         & LLM4OM + MPT-7B            & 89.70 & 20.19 & 32.97        \\ \hline
  %       \bottomrule
  %     \end{tabular}
  %   }
  %   \subcaption{Performance of KROMA compared to state-of-the-art LLM-based ontology matching systems and variations.}
  %   \label{tab:sub:h_others}
  % \end{subtable}
  \begin{subtable}[t]{\linewidth}
  \centering
  \scriptsize
  \setlength{\tabcolsep}{2pt}
  \begin{tabular}{l l c c c}
    \toprule
    \textbf{Dataset} & \textbf{Model} & \textbf{$P$} & \textbf{$R$} & \textbf{$F_1$} \\
    \midrule
    \multirow{8}{*}{Mouse-Human}
      & KL3.3 & 90.78 & 99.50 & \textbf{94.94} \\
      & KNR3.3 & 92.34 & 90.16 & 91.25 \\
      & KNB3.3 &100.00 & 76.36 & 86.59 \\
      & KL3.1 & 90.42 & 99.00 & 94.50 \\
      & KL2.0 &100.00 & 87.34 & 93.24 \\
      & ML3.1 &100.00 & 87.50 & 92.20 \\
      & OL2.0 & 91.40 & 89.10 & 90.20 \\
      & L4G3.5 & 90.82 & 87.46 & 89.11 \\
    \midrule
    \multirow{8}{*}{NCIT-DOID}
      & KL3.3 & 97.59 & 99.69 & \textbf{98.63} \\
      & KNR3.3 & 93.20 & 96.90 & 95.01 \\
      & KNB3.3 & 83.33 &100.00 & 90.91 \\
      & KL3.1 & 97.43 & 99.08 & 98.24 \\
      & KG2   & 66.67 &100.00 & 80.00 \\
      & ML3.1 & 96.40 & 93.20 & 94.80 \\
      & LLFT  & 86.10 & 62.00 & 72.10 \\
      & L4G3.5 & 86.19 & 80.06 & 83.01 \\
    \midrule
    \multirow{6}{*}{Nell-DBpedia}
      & KL3.3 & 94.32 &100.00 & \textbf{97.08} \\
      & KNR3.3 & 97.46 & 91.27 & 94.26 \\
      & KNB3.3 & 91.17 & 96.12 & 93.58 \\
      & KL2.0 & 95.50 & 96.55 & 96.02 \\
      & OL2.0 &100.00 & 92.20 & 96.00 \\
      & L4G3.5 &100.00 & 89.14 & 94.26 \\
    \midrule
    \multirow{5}{*}{YAGO-Wikidata}
      & KL3.3 & 91.80 & 99.60 & 95.54 \\
      & KNR3.3 & 93.50 & 90.50 & 91.98 \\
      & KNB3.3 & 90.50 & 89.00 & 89.74 \\
      & KL3.2 & 89.09 & 98.00 & 93.33 \\
      & L4L2  &100.00 & 85.52 & 92.19 \\
    \midrule
    \multirow{9}{*}{ENVO-SWEET}
      & K4mini & 87.23 &100.00 & \textbf{93.18} \\
      & KNR4mini &86.90 & 98.00 & 92.12 \\
      & KNB4mini &82.00 & 88.00 & 84.89 \\
      & KL3.1  & 87.11 & 96.19 & 91.43 \\
      & KL2.0  & 92.50 & 78.72 & 85.06 \\
      & KM7    & 87.19 & 99.59 & 92.98 \\
      & ML3.1  & 80.30 & 59.50 & 83.70 \\
      & OL2.0  & 43.10 & 61.30 & 51.10 \\
      & L4M7   & 59.00 & 51.67 & 55.09 \\
    \midrule
    \multirow{5}{*}{MI-MatOnto}
      & KL3.3  & 45.74 & 92.69 & \textbf{61.25} \\
      & KNR3.3 & 44.80 & 91.40 & 59.95 \\
      & KNB3.3 & 42.00 & 85.00 & 55.00 \\
      & KL3.2  & 56.36 & 62.00 & 59.05 \\
      & L4MPT  & 89.70 & 20.19 & 32.97 \\
    \bottomrule
  \end{tabular}
  \subcaption{All systems (codes) across 6 datasets.}
  \label{tab:sub:all_codes}
\end{subtable}
\end{table}

\begin{table}[!htb]
  \centering
  %% (g) Scalability
  \begin{subtable}[t]{\linewidth}
    \centering
    \begin{tabular}{l l c c c}
      \toprule
      {\bfseries Dataset}      & {\bfseries Data Size} & {\bfseries $P$} & {\bfseries $R$} & {\bfseries $F_1$} \\ \midrule
      \multirow{5}{*}{NCIT-DOID}
        & xsmall & 97.50 & 97.50 & 97.50 \\
        & small  & 97.88 & 98.12 & 98.00 \\
        & medium & 97.92 & 97.50 & 97.71 \\
        & large  & 98.00 & 98.13 & 98.06 \\
        & full   & 97.59 & 99.69 & 98.63 \\ \midrule
      \multirow{5}{*}{Nell-DBpedia}
        & xsmall & 95.00 & 96.67 & 95.83 \\
        & small  & 95.19 & 98.33 & 96.74 \\
        & medium & 95.24 & 99.17 & 97.18 \\
        & large  & 95.63 & 99.58 & 97.58 \\
        & full   & 94.32 & 100.00 & 97.08 \\ \midrule
      \multirow{5}{*}{YAGO-Wikidata}
        & xsmall & 92.00 & 98.00 & 94.90 \\
        & small  & 92.50 & 98.75 & 95.58 \\
        & medium & 92.67 & 99.17 & 95.89 \\
        & large  & 92.75 & 99.38 & 96.04 \\
        & full   & 91.80 & 99.60 & 95.54 \\ \bottomrule
    \end{tabular}
    \subcaption{Scale: performance across ontology sizes.}
    \label{tab:sub:g_scale}
  \end{subtable}
    %% (c) API Call Reduction
  \begin{subtable}[t]{\linewidth}
    \centering
    \begin{tabular}{|l|r|r|r|}
      \hline
      \textbf{Dataset}      & \textbf{Qwen2.5-1.5B} & \textbf{GPT-4o-mini} & \textbf{Llama-3.3-70B} \\ \hline
      Mouse-Human          & 3.06\%  & 2.88\%  & 6.76\%  \\ \hline
      NCIT-DOID            & 54.48\% & 54.63\% & 54.48\% \\ \hline
      Nell-DBpedia         & 26.09\% & 25.76\% & 26.09\% \\ \hline
      YAGO-Wikidata        & 21.86\% & 21.93\% & 22.01\% \\ \hline
      ENVO-SWEET           & 6.99\%  & 6.82\%  & 6.99\%  \\ \hline
      MI-MatOnto           & 43.04\% & 41.66\% & 41.81\% \\ \hline
      \textbf{ALL}         & \textbf{25.92\%} & \textbf{25.61\%} & \textbf{26.36\%} \\ \hline
    \end{tabular}
    \subcaption{API Call Reduction (\%) by dataset and model.}
    \label{tab:sub:c_api}
  \end{subtable}
\end{table}

\begin{table}[!htb]
  \centering
  %% (d) LLM Debate
  \begin{subtable}[t]{\linewidth}
    \centering
    \begin{tabular}{|l|l|c|c|c|c|}
      \hline
      {\bfseries Dataset} & {\bfseries Model}   & {\bfseries $P$} & {\bfseries $R$} & {\bfseries $F_1$} & {\bfseries OM-LLM} \\ \hline
      \multirow{4}{*}{Mouse-Human}
        & Debate-2A-3R       & 100   & 70    & 82.35 & \multirow{4}{*}{92.20} \\
        & Debate-2A-5R       & 100   & 74    & 85.06 &                         \\
        & Debate-4A-3R       & 100   & 66    & 79.52 &                         \\
        & Debate-4A-5R       & 100   & 68    & 80.95 &                         \\ \hline
      \multirow{4}{*}{Nell-DBpedia}
        & Debate-2A-3R       & 97.83 & 90    & 93.75 & \multirow{4}{*}{96}    \\
        & Debate-2A-5R       & 95.91 & 94    & 94.95 &                         \\
        & Debate-4A-3R       & 95.55 & 86    & 90.53 &                         \\
        & Debate-4A-5R       & 93.88 & 92    & 92.93 &                         \\ \hline
      \multirow{4}{*}{YAGO-Wikidata}
        & Debate-2A-3R       & 100   & 92    & 95.83 & \multirow{4}{*}{92.19} \\
        & Debate-2A-5R       & 100   & 96.88 & 98.41 &                         \\
        & Debate-4A-3R       & 100   & 86    & 92.47 &                         \\
        & Debate-4A-5R       & 100   & 90    & 94.73 &                         \\ \hline
    \end{tabular}
    \subcaption{LLM Debate on zero-shot matching performance.}
    \label{tab:sub:d_debate}
  \end{subtable}

  \vspace{1ex}

  %% (e) Long vs. Short Chain-of-Thought
  \begin{subtable}[t]{\linewidth}
    \centering
    \begin{tabular}{|l|l|c|c|c|c|}
      \hline
      {\bfseries Dataset}    & {\bfseries Model}           & {\bfseries $P$} & {\bfseries $R$} & {\bfseries $F_1$} & {\bfseries OM-LLM} \\ \hline
      \multirow{2}{*}{NCIT-DOID}
        & Llama-3.3-70B        & 97.59 & 99.69 & 98.63 & \multirow{2}{*}{94.80} \\
        & DR1D-Llama-3.3-70B   & 97.66 & 96.31 & 96.98 &                         \\ \hline
      \multirow{2}{*}{Nell-DBpedia}
        & Llama-3.3-70B        & 94.32 & 100.00 & 97.08 & \multirow{2}{*}{96}    \\
        & DR1D-Llama-3.3-70B   & 94.67 & 95.48  & 95.07 &                         \\ \hline
      \multirow{2}{*}{YAGO-Wikidata}
        & Llama-3.3-70B        & 91.80 & 99.60 & 95.54 & \multirow{2}{*}{92.19} \\
        & DR1D-Llama-3.3-70B   & 92.31 & 94.80 & 93.53 &                         \\ \hline
    \end{tabular}
    \subcaption{Performance of short vs. long reasoning LLMs.}
    \label{tab:sub:e_longshort}
  \end{subtable}

  \vspace{1ex}

  %% (f) Active Learning
  \begin{subtable}[t]{\linewidth}
    \centering
    \begin{tabular}{|l|l|c|c|c|}
      \hline
      {\bfseries Dataset}     & {\bfseries Model}           & {\bfseries $P$} & {\bfseries $R$} & {\bfseries $F_1$} \\ \hline
      \multirow{2}{*}{NCIT-DOID}
        & KROMA + Llama-3.1-70B & 97.85 & 98.15 & \textbf{98} \\
        & MILA + Llama-3.1-70B  & 96.70 & 92.80 & 94.67      \\ \hline
    \end{tabular}
    \subcaption{Active learning on NCIT-DOID.}
    \label{tab:sub:f_active}
  \end{subtable}

  \caption{All benchmark and evaluation tables combined into a single multi‐subtable float.}
  \label{tab:all_subtables}
\end{table}

==> assets/old_tables.tex <==
\begin{table}[h!]
\centering
\begin{tabular}{lcc}
\hline
\textbf{Model} & \textbf{Parameters} & \textbf{MMLU Score (\%)} \\
\hline
Gemma-2B & 2B & 51.3 \\
Flan-T5-XXL & 11B & 55.1 \\
Llama-3.2-3B & 3B & 63.4 \\
Llama-2-7B & 7B & 68.9 \\
Mistral-7B & 7B & 60.1 \\
\hline
\end{tabular}
\caption{Benchmark comparison of models based on MMLU (5-shot, top-1).}
\label{tab:mmlu_comparison}
\end{table}

% -------- KROMA_MODELS --------
\begin{table}[!htbp]
  \centering
  % \scriptsize                     % smaller font
  \setlength{\tabcolsep}{3pt}     % tighter columns
  \label{tab:kroma_models}
  \resizebox{\textwidth}{!}{%
    \begin{tabular}{ll
        *{3}{ccc}   % three KROMA blocks
        |ccc         % vertical line + OM‑LLM P,R,$F_1$
      }
      \toprule
      \multicolumn{2}{c}{\bfseries Task / Model} &
        \multicolumn{3}{c}{\bfseries Qwen2.5‑1.5B} &
        \multicolumn{3}{c}{\bfseries GPT‑4o‑mini} &
        \multicolumn{3}{c}{\bfseries Llama‑3.3‑70B} &
        \multicolumn{3}{c}{\bfseries OM‑LLM} \\
      \cmidrule(lr){1-2} \cmidrule(lr){3-5}
      \cmidrule(lr){6-8} \cmidrule(lr){9-11}
      \cmidrule(lr){12-14}
      {\bfseries Task} &  & P & R & $F_1$ & P & R & $F_1$ & P & R & $F_1$ & P & R & $F_1$ \\
      \midrule
      Mouse‑Human
        &          & 84.66 & 82.52 & 83.58 & 85.12 & 100 & 91.96 & 90.78 & 99.50 & \textbf{94.94} & 97.40 & 87.50  & 92.20 \\
      NCIT‑DOID
        &          & 95.00 & 100.00 & \bfseries97.44 & 95.24 & 100.00 & \bfseries97.56 & 97.59 & 99.69 & \bfseries98.63 & 96.40     & 93.20     & 94.80 \\
      Nell‑DBpedia
        &          & 96.30 & 94.10 & 95.02 & 95.89 & 95.64 & 95.67 & 94.32 & 100.00 & \textbf{97.08} & 100     & 92.20     & 96.00 \\
      YAGO‑Wikidata
        &          & 93.81 & 97.15 & \bfseries95.45 & 93.79 & 97.14 & \bfseries95.44 & 91.80 & 99.60 & \bfseries95.54 & 100     & 85.52     & 92.19 \\
      ENVO‑SWEET
        &           & 87.37   & 73.45   & 79.80 & 87.23   & 100   & \textbf{93.18} & 87.16   & 97.29   & \textbf{91.95} & 80.30     & 59.50     & 83.70 \\
      MI‑MatOnto
        &          & 45.74 & 92.69 & \bfseries61.25 & 46.08 & 89.70 & \bfseries60.88 & 46.68 & 93.36 & \bfseries62.24 & 89.70     & 20.19     & 32.97 \\
      \bottomrule
    \end{tabular}%
  }
  \caption{Zero‑shot performance across six tasks using three LLMs. Bold $F_1$ indicates where KROMA beats the best existing OM‑LLM.}
\end{table}

% -------- API REDUCE --------
\begin{table}[!htbp]
\centering
% \small
% \setlength{\tabcolsep}{4pt} % Adjust horizontal padding between columns
\label{tab:api_call_reduce}
\begin{tabular}{|l|r|r|r|}
\hline
\textbf{Dataset}       & \textbf{Qwen2.5-1.5B} & \textbf{GPT-4o-mini} & \textbf{Llama-3.3-70B} \\ 
\hline
Mouse-Human    & 3.06\%  & 2.88\%  & 6.76\%  \\ \hline
NCIT-DOID      & 54.48\%  & 54.63\%  & 54.48\%  \\ \hline
Nell-DBpedia   & 26.09\%  & 25.76\%  & 26.09\%  \\ \hline
YAGO-Wikidata  & 21.86\% & 21.93\% & 22.01\% \\ \hline
ENVO-SWEET     & 6.99\%  & 6.82\%  & 6.99\%  \\ \hline
MI-MatOnto     & 43.04\% & 41.66\% & 41.81\% \\ \hline
\textbf{ALL}    & \textbf{25.92\%} & \textbf{25.61\%} & \textbf{26.36\%} \\ 
\hline
\end{tabular}
\caption{API Call Reduction (\%) by Dataset and Model}
\end{table}
% ----------------------------

% -------- LLM DEBATE --------
\begin{table}[!htbp]
\centering
\label{tab:kroma_llm_debate}
\begin{tabular}{|l|l|c|c|c|c|}
\hline
{\bfseries Dataset} & {\bfseries Model} & {\bfseries P} & {\bfseries R} & {\bfseries $F_1$} & \bfseries OM-LLM \\
\hline
\multirow{4}{*}{Mouse-Human} 
    & Debate-2A-3R   & 100   & 70  & 82.35   & \multirow{4}{*}{92.20}  \\
    & Debate-2A-5R   & 100   & 74  & 85.06   &  \\
    & Debate-4A-3R   & 100   & 66  & 79.52   &  \\
    & Debate-4A-5R   & 100   & 68  & 80.95   &  \\
\hline

\multirow{4}{*}{Nell-DBpedia} 
    & Debate‑2A‑3R   & 97.83   & 90  & 93.75   & \multirow{4}{*}{96} \\
    & Debate‑2A‑5R   & 95.91   & 94  & 94.95   &  \\
    & Debate‑4A‑3R   & 95.55   & 86  & 90.53   &  \\
    & Debate‑4A‑5R   & 93.88   & 92  & 92.93   &  \\
\hline

\multirow{4}{*}{YAGO-Wikidata} 
    & Debate‑2A‑3R   & 100   & 92  & 95.83   & \multirow{4}{*}{92.19} \\
    & Debate‑2A‑5R   & 100   & 96.88  & 98.41   &  \\
    & Debate‑4A‑3R   & 100   & 86  & 92.47   &  \\
    & Debate‑4A‑5R   & 100   & 90  & 94.73   &  \\
\hline

\end{tabular}
\caption{LLM Debate on Zero‑Shot Matching Performance on Anatomy's Mouse‑Human dataset. 4 settings are considered: 2/3 Agents and 3/5 Rounds. The “OM‑LLM” column reports the highest $F_1$ score achieved by any current LLM‑based OM system.}
\end{table}
% ----------------------------

% -------- LONG SHORT --------
\begin{table}[!htbp]
\centering
\label{tab:longshort_result}
\begin{tabular}{|l|l|c|c|c|c|}
\hline
{\bfseries Datasets} & {\bfseries Model} & {\bfseries Precision} & {\bfseries Recall} & {\bfseries $F_1$} & \multicolumn{1}{c|}{\bfseries OM-LLM} \\
\hline
\multirow{2}{*}{NCIT-DOID} 
    & Llama-3.3-70B           & 97.59 & 99.69 & 98.63   & \multirow{2}{*}{94.80} \\
    & DR1D-Llama-3.3-70B      & 97.66   & 96.31      & 96.98   &  \\
\hline
\multirow{2}{*}{Nell-DBPedia} 
    & Llama-3.3-70B           & 94.32 & 100.00 & 97.08   & \multirow{2}{*}{96} \\
    & DR1D-Llama-3.3-70B      & 94.67   & 95.48      & 95.07   &  \\
\hline
\multirow{2}{*}{YAGO-Wikidata} 
    & Llama-3.3-70B           & 91.80 & 99.60 & 95.54   & \multirow{2}{*}{92.19} \\
    & DR1D-Llama-3.3-70B      & 92.31   & 94.8      & 93.53   &  \\
\hline
\end{tabular}
\caption{Performance of Short and Long Reasoning LLMs on Anatomy's Mouse–Human Dataset. The “OM‑LLM” column reports the highest $F_1$ score achieved by any current LLM‑based OM system.}
\end{table}
% ----------------------------

% -------- ACTIVE LEARNING --------
\begin{table}[!htbp]
\centering
\label{tab:active_learning}
\begin{tabular}{|l|l|c|c|c|}
\hline
{\bfseries Datasets} & {\bfseries Model} & {\bfseries Precision} & {\bfseries Recall} & {\bfseries $F_1$} \\
\hline
\multirow{2}{*}{NCIT-DOID} 
    & KROMA + Llama-3.1-70B  & 97.85   & 98.15     & \textbf{98} \\
    & MILA + Llama-3.1-70B   & 96.70   & 92.80      & 94.67 \\
\hline
\end{tabular}
\caption{Active Learning}
\end{table}
% ----------------------------

% % -------- SCALABILITY --------
\begin{table}[!htbp]
\centering
\label{tab:scale}
\begin{tabular}{l l c c c}
\toprule
{\bfseries Dataset}      & {\bfseries Data Size} & {\bfseries P}   & {\bfseries R}   & {\bfseries $F_1$}  \\
\midrule

\multirow{5}{*}{NCIT-DOID} 
    & xsmall & 97.50 & 97.50 & 97.50 \\ % TP=78/80, FP=2, FN=2, TN=118
    & small  & 97.88 & 98.12 & 98.00 \\ % TP=157/160, FP=3, FN=3, TN=237
    & medium   & 97.92 & 97.50 & 97.71 \\ % TP=234/240, FP=5, FN=6, TN=355
    & large  & 98.00 & 98.13 & 98.06 \\ % TP=313/320, FP=6, FN=7, TN=474
    & full     & 97.59 & 99.69 & 98.63 \\
\midrule

\multirow{5}{*}{Nell-DBpedia} 
    & xsmall   & 95.00 & 96.67 & 95.83 \\ % TP=58/60, FP=3, FN=2, TN=137
    & small   & 95.19 & 98.33 & 96.74 \\ % TP=118/120, FP=6, FN=2, TN=274
    & medium   & 95.24 & 99.17 & 97.18 \\ % TP=178/180, FP=9, FN=2, TN=411
    & large   & 95.63 & 99.58 & 97.58 \\ % TP=239/240, FP=11, FN=1, TN=549
    & full     & 94.32 & 100.00 & 97.08 \\
\midrule

\multirow{5}{*}{YAGO-Wikidata} 
    & xsmall   & 92.00 & 98.00 & 94.90 \\ % TP=49/50, FP=4, FN=1, TN=146
    & small  & 92.50 & 98.75 & 95.58 \\ % TP=79/80, FP=6, FN=1, TN=234
    & medium   & 92.67 & 99.17 & 95.89 \\ % TP=149/150, FP=12, FN=1, TN=438
    & large   & 92.75 & 99.38 & 96.04 \\ % TP=199/200, FP=16, FN=1, TN=584
    & full     & 91.80 & 99.60 & 95.54 \\
\bottomrule
\end{tabular}
\caption{Scale.}
\end{table}
% % ----------------------------

% -------- KROMA AND OTHERS --------
\begin{table}[!htbp]
\centering
\label{tab:kroma_and_others}
\resizebox{\textwidth}{!}{%
\begin{tabular}{|l|l|c|c|c|}
\hline
{\bfseries Dataset} & {\bfseries Model} & {\bfseries P} & {\bfseries R} & {\bfseries $F_1$} \\
\hline

\multirow{8}{*}{Mouse-Human} 
    & KROMA + Llama-3.3-70B     & 90.78 & 99.50 & \textbf{94.94}   \\
    & KROMA-NR + Llama-3.3-70B   & 92.34 & 90.16 & 91.25   \\
    & KROMA-NB + Llama-3.3-70B   & 100   & 76.36   & 86.59  \\
    & KROMA + Llama-3.1-70B  & 90.42   & 99.00   & \textbf{94.50}  \\
    & KROMA + Llama-2-70B  & 100   & 87.34   & \textbf{93.24}  \\
    & MILA + Llama-3.1-70B    & 100   & 87.50   & 92.20   \\
    & OLaLa + Llama-2-70B    & 91.40   & 89.10   & 90.20   \\
    & LLM4OM + GPT-3.5-175B       & 90.82   & 87.46   & 89.11   \\
\hline

\multirow{8}{*}{NCIT-DOID} 
    & KROMA + Llama-3.3-70B      & 97.59   & 99.69  & \textbf{98.63}  \\
    & KROMA-NR + Llama-3.3-70B  & 93.20   & 96.90   & \textbf{95.01}  \\
    & KROMA-NB + Llama-3.3-70B  & 83.33   & 100   & 90.91  \\
    & KROMA + Llama-3.1-70B  & 97.43   & 99.08   & 98.24  \\
    & KROMA + Gemma-2B  & 66.67   & 100   & 80  \\
    & MILA + Llama-3.1-70B      & 96.40   & 93.20   & 94.80  \\
    & LLMap + Flan-T5-XXL      & 86.10   & 62.00   & 72.10  \\
    & LLM4OM + GPT-3.5-175B         & 86.19   & 80.06   & 83.01  \\
\hline

\multirow{6}{*}{Nell-DBpedia} 
    & KROMA + Llama-3.3-70B  & 94.32 & 100.00 & \textbf{97.08}  \\
    & KROMA-NR + Llama-3.3-70B  & 97.46 & 91.27 & 94.26  \\
     & KROMA-NB + Llama-3.3-70B  & 91.17   & 96.12   & 93.58  \\
    & KROMA + Llama-2-70B   & 95.50   & 96.55   & \textbf{96.02}  \\
    & OLaLa + Llama-2-70B      & 100   & 92.20   & 96   \\
    & LLM4OM + GPT-3.5-175B & 100   & 89.14   & 94.26  \\
\hline

\multirow{5}{*}{YAGO-Wikidata} 
    & KROMA + Llama-3.3-70B      & 91.80 & 99.60 & 95.54   \\
    & KROMA‑NR + Llama-3.3-70B   & 93.50   & 90.50   & 91.98   \\
    & KROMA‑NB + Llama-3.3-70B   & 90.50   & 89.00   & 89.74   \\
    & KROMA + Llama-3.2-3B      &  89.09  & 98   & 93.33   \\
    & LLM4OM + Llama‑2‑7B       & 100.00  & 85.52   & 92.19           \\
\hline

\multirow{9}{*}{ENVO-SWEET} 
    & KROMA + GPT-4o-mini       & 87.23   & 100.00   & \textbf{93.18}   \\
    & KROMA-NR + GPT-4o-mini    & 86.90   &  98.00   & 92.12   \\
    & KROMA-NB + GPT-4o-mini    & 82.00   &  88.00   & 84.89   \\
    & KROMA + Llama-3.1-70B     & 87.11   &  96.19   & 91.43   \\
    & KROMA + Llama-2-70B       &   92.50     &    78.72     &   85.06     \\
    & KROMA + Mistral-7B        & 87.19   &  99.59   & 92.98   \\
    & MILA + Llama-3.1-70B      & 80.30   &  59.50   & 83.70   \\
    & OLaLa + Llama-2-70B       & 43.10   &  61.30   & 51.10   \\
    & LLM4OM + Mistral-7B       & 59.00   &  51.67   & 55.09   \\
\hline


\multirow{5}{*}{MI-MatOnto} 
    & KROMA + Llama-3.3-70B      & 45.74   & 92.69   & \textbf{61.25}   \\
    & KROMA-NR + Llama-3.3-70B   & 44.80   & 91.40   & 59.95   \\
    & KROMA-NB + Llama-3.3-70B   & 42.00   & 85.00   & 55.00   \\
    & KROMA + Llama-3.2-3B            &  56.36      &  62      &  59.05      \\
    & LLM4OM + MPT-7B            & 89.70   & 20.19   & 32.97   \\
\hline
\end{tabular}
}
\caption{Performance of KROMA compared to state‑of‑the‑art LLM‑based ontology matching systems and variations of KROMA across six benchmark datasets. Bolded $F_1$ values denote cases where KROMA outperforms the best existing LLM‑based OM system.}
\end{table}
% ----------------------------

\begin{table}[!htbp]
\centering
\small
\label{tab:model_codes}
\begin{tabular}{llll}
\toprule
\textbf{Code}   & \textbf{System} & \textbf{Variant} & \textbf{Version}       \\
\midrule
KL3.3    & KROMA    & –   & Llama-3.3-70B   \\
KNR3.3   & KROMA    & NR  & Llama-3.3-70B   \\
KNB3.3   & KROMA    & NB  & Llama-3.3-70B   \\
KL3.1    & KROMA    & –   & Llama-3.1-70B   \\
KL2.0    & KROMA    & –   & Llama-2-70B     \\
ML3.1    & MILA     & –   & Llama-3.1-70B   \\
OL2.0    & OLaLa    & –   & Llama-2-70B     \\
L4G3.5   & LLM4OM   & –   & GPT-3.5-175B    \\
K4mini   & KROMA    & –   & GPT-4o-mini     \\
KNR4mini & KROMA    & NR  & GPT-4o-mini     \\
KNB4mini & KROMA    & NB  & GPT-4o-mini     \\
KG2      & KROMA    & –   & Gemma-2B        \\
LLFT     & LLMap    & –   & Flan-T5-XXL     \\
KM7      & KROMA    & –   & Mistral-7B      \\
L4M7     & LLM4OM   & –   & Mistral-7B      \\
KL3.2    & KROMA    & –   & Llama-3.2-3B    \\
L4L2     & LLM4OM   & –   & Llama-2-7B      \\
L4MPT    & LLM4OM   & –   & MPT-7B          \\
\bottomrule
\end{tabular}
\caption{Abbreviation mapping for model codes}
\end{table}

==> assets/tables.tex <==
\begin{table}[!htb]
  \centering
  \setlength{\tabcolsep}{3pt}
  \resizebox{\textwidth}{!}{%
    \begin{tabular}{ll *{3}{ccc} |ccc}
      \toprule
      \multicolumn{2}{c}{\bfseries Task / Model} &
        \multicolumn{3}{c}{\bfseries Qwen2.5-1.5B} &
        \multicolumn{3}{c}{\bfseries GPT-4o-mini} &
        \multicolumn{3}{c}{\bfseries Llama-3.3-70B} &
        \multicolumn{3}{c}{\bfseries OM-LLM} \\
      \cmidrule(lr){1-2} \cmidrule(lr){3-5}
      \cmidrule(lr){6-8} \cmidrule(lr){9-11}
      \cmidrule(lr){12-14}
      {\bfseries Task} & & $P$ & $R$ & $F_1$ & $P$ & $R$ & $F_1$ & $P$ & $R$ & $F_1$ & $P$ & $R$ & $F_1$ \\
      \midrule
      Mouse-Human   & & 84.66 & 82.52 & 83.58 & 85.12 & 100.00 & 91.96 & 90.78  & 99.50 & \textbf{94.94} & 97.40 & 87.50 & 92.20 \\
      NCIT-DOID     & & 95.00 & 100.00 & \bfseries97.44 & 95.24 & 100.00 & \bfseries97.56 & 97.59 & 99.69 & \bfseries98.63 & 96.40 & 93.20 & 94.80 \\
      Nell-DBpedia  & & 96.30 & 94.10  & 95.02          & 95.89 & 95.64  & 95.67          & 94.32 & 100.00 & \textbf{97.08} & 100.00 & 92.20 & 96.00 \\
      YAGO-Wikidata & & 93.81 & 97.15  & \bfseries95.45  & 93.79 & 97.14  & \bfseries95.44  & 91.80 & 99.60  & \bfseries95.54  & 100.00 & 85.52 & 92.19 \\
      ENVO-SWEET    & & 87.37 & 73.45  & 79.80          & 87.23 & 100.00 & \textbf{93.18} & 87.16 & 97.29  & \textbf{91.95} & 80.30 & 59.50 & 83.70 \\
      MI-MatOnto    & & 45.74 & 92.69  & \bfseries61.25  & 46.08 & 89.70  & \bfseries60.88  & 46.68 & 93.36  & \bfseries62.24  & 89.70 & 20.19 & 32.97 \\
      \bottomrule
    \end{tabular}%
  }
  \caption{Performance across six tasks using three LLMs. Bold $F_1$ indicates where KROMA beats the best existing OM-LLM.}
  \label{tab:b_kroma}
\end{table}

\begin{table}[!htb]
  \centering
  \begin{tabular}{llll}
    \toprule
    \textbf{Code} & \textbf{System} & \textbf{Variant} & \textbf{Version} \\ 
    \midrule
    KL3.3     & KROMA  & –  & Llama-3.3-70B   \\
    KNR3.3    & KROMA  & NR & Llama-3.3-70B   \\
    KNB3.3    & KROMA  & NB & Llama-3.3-70B   \\
    KNB3.2    & KROMA  & NB & Llama-3.2-3B    \\
    KL3.1     & KROMA  & –  & Llama-3.1-70B   \\
    KL2.0     & KROMA  & –  & Llama-2-70B     \\
    K4mini    & KROMA  & –  & GPT-4o-mini     \\
    KNR4mini  & KROMA  & NR & GPT-4o-mini     \\
    KNB4mini  & KROMA  & NB & GPT-4o-mini     \\
    KG2       & KROMA  & –  & Gemma-2B        \\
    KM7       & KROMA  & –  & Mistral-7B      \\
    ML3.1     & MILA   & –  & Llama-3.1-70B   \\
    OL2.0     & OLaLa  & –  & Llama-2-70B     \\
    L4G3.5    & LLM4OM & –  & GPT-3.5-175B    \\
    L4L2      & LLM4OM & –  & Llama-2-7B      \\
    L4MPT     & LLM4OM & –  & MPT-7B          \\
    LLFT      & LLM4OM & –  & Flan-T5-XXL     \\
    \bottomrule
  \end{tabular}
  \caption{Abbreviation mapping for model codes.}
  \label{tab:codes}
\end{table}

\begin{table}[!htb]
  \centering
  \begin{tabular}{lcc}
    \toprule
    \textbf{Model}       & \textbf{Parameters} & \textbf{MMLU Score (\%)} \\
    \midrule
    Gemma-2B         & 2B  & 51.3 \\
    Flan-T5-XXL      & 11B & 55.1 \\
    Llama-3.2-3B     & 3B  & 63.4 \\
    Llama-2-7B       & 7B  & 68.9 \\
    Mistral-7B       & 7B  & 60.1 \\
    \bottomrule
  \end{tabular}
  \caption{Benchmark comparison of models based on MMLU (5-shot, top-1).}
  \label{tab:a_mmlu}
\end{table}

\begin{table}[!ht]
  \centering
  \scriptsize
  \setlength{\tabcolsep}{2pt}
  \begin{tabular}{l l c c c}
    \toprule
    \textbf{Dataset} & \textbf{Model} & \textbf{$P$} & \textbf{$R$} & \textbf{$F_1$} \\
    \midrule
    \multirow{8}{*}{Mouse-Human}
      & KL3.3   & 90.78 & 99.50 & \textbf{94.94} \\
      & KNR3.3  & 92.34 & 90.16 & 91.25 \\
      & KNB3.3  &100.00 & 76.36 & 86.59 \\
      & KL3.1   & 90.42 & 99.00 & 94.50 \\
      & KL2.0   &100.00 & 87.34 & 93.24 \\
      & ML3.1   &100.00 & 87.50 & 92.20 \\
      & OL2.0   & 91.40 & 89.10 & 90.20 \\
      & L4G3.5  & 90.82 & 87.46 & 89.11 \\
    \midrule
    \multirow{8}{*}{NCIT-DOID}
      & KL3.3   & 97.59 & 99.69 & \textbf{98.63} \\
      & KNR3.3  & 93.20 & 96.90 & 95.01 \\
      & KNB3.3  & 83.33 &100.00 & 90.91 \\
      & KL3.1   & 97.43 & 99.08 & 98.24 \\
      & KG2     & 66.67 &100.00 & 80.00 \\
      & ML3.1   & 96.40 & 93.20 & 94.80 \\
      & LLFT    & 86.10 & 62.00 & 72.10 \\
      & L4G3.5  & 86.19 & 80.06 & 83.01 \\
    \midrule
    \multirow{6}{*}{Nell-DBpedia}
      & KL3.3   & 94.32 &100.00 & \textbf{97.08} \\
      & KNR3.3  & 97.46 & 91.27 & 94.26 \\
      & KNB3.3  & 91.17 & 96.12 & 93.58 \\
      & KL2.0   & 95.50 & 96.55 & 96.02 \\
      & OL2.0   &100.00 & 92.20 & 96.00 \\
      & L4G3.5  &100.00 & 89.14 & 94.26 \\
    \midrule
    \multirow{5}{*}{YAGO-Wikidata}
      & KL3.3   & 91.80 & 99.60 & 95.54 \\
      & KNR3.3  & 93.50 & 90.50 & 91.98 \\
      & KNB3.3  & 90.50 & 89.00 & 89.74 \\
      & KL3.2   & 89.09 & 98.00 & 93.33 \\
      & L4L2    &100.00 & 85.52 & 92.19 \\
    \midrule
    \multirow{9}{*}{ENVO-SWEET}
      & K4mini  & 87.23 &100.00 & \textbf{93.18} \\
      & KNR4mini& 86.90 & 98.00 & 92.12 \\
      & KNB4mini& 82.00 & 88.00 & 84.89 \\
      & KL3.1   & 87.11 & 96.19 & 91.43 \\
      & KL2.0   & 92.50 & 78.72 & 85.06 \\
      & KM7     & 87.19 & 99.59 & 92.98 \\
      & ML3.1   & 80.30 & 59.50 & 83.70 \\
      & OL2.0   & 43.10 & 61.30 & 51.10 \\
      & L4M7    & 59.00 & 51.67 & 55.09 \\
    \midrule
    \multirow{5}{*}{MI-MatOnto}
      & KL3.3   & 45.74 & 92.69 & \textbf{61.25} \\
      & KNR3.3  & 44.80 & 91.40 & 59.95 \\
      & KNB3.3  & 42.00 & 85.00 & 55.00 \\
      & KL3.2   & 56.36 & 62.00 & 59.05 \\
      & L4MPT   & 89.70 & 20.19 & 32.97 \\
    \bottomrule
  \end{tabular}
  \caption{All systems (codes) across 6 datasets.}
  \label{tab:all_codes}
\end{table}

\begin{table}[!htb]
  \centering
  \begin{tabular}{l l c c c}
    \toprule
    {\bfseries Dataset}      & {\bfseries Data Size} & {\bfseries $P$} & {\bfseries $R$} & {\bfseries $F_1$} \\ 
    \midrule
    \multirow{5}{*}{NCIT-DOID}
      & xsmall & 97.50 & 97.50 & 97.50 \\
      & small  & 97.88 & 98.12 & 98.00 \\
      & medium & 97.92 & 97.50 & 97.71 \\
      & large  & 98.00 & 98.13 & 98.06 \\
      & full   & 97.59 & 99.69 & 98.63 \\
    \midrule
    \multirow{5}{*}{Nell-DBpedia}
      & xsmall & 95.00 & 96.67 & 95.83 \\
      & small  & 95.19 & 98.33 & 96.74 \\
      & medium & 95.24 & 99.17 & 97.18 \\
      & large  & 95.63 & 99.58 & 97.58 \\
      & full   & 94.32 &100.00 & 97.08 \\
    \midrule
    \multirow{5}{*}{YAGO-Wikidata}
      & xsmall & 92.00 & 98.00 & 94.90 \\
      & small  & 92.50 & 98.75 & 95.58 \\
      & medium & 92.67 & 99.17 & 95.89 \\
      & large  & 92.75 & 99.38 & 96.04 \\
      & full   & 91.80 & 99.60 & 95.54 \\
    \bottomrule
  \end{tabular}
  \caption{Scale: performance across ontology sizes.}
  \label{tab:g_scale}
\end{table}

\begin{table}[!htb]
  \centering
  \begin{tabular}{|l|r|r|r|}
    \hline
    \textbf{Dataset}      & \textbf{Qwen2.5-1.5B} & \textbf{GPT-4o-mini} & \textbf{Llama-3.3-70B} \\ 
    \hline
    Mouse-Human   & 3.06\%  & 2.88\%  & 6.76\%  \\ 
    NCIT-DOID     & 54.48\% & 54.63\% & 54.48\% \\ 
    Nell-DBpedia  & 26.09\% & 25.76\% & 26.09\% \\ 
    YAGO-Wikidata & 21.86\% & 21.93\% & 22.01\% \\ 
    ENVO-SWEET    & 6.99\%  & 6.82\%  & 6.99\%  \\ 
    MI-MatOnto    & 43.04\% & 41.66\% & 41.81\% \\ 
    \hline
    \textbf{ALL}         & \textbf{25.92\%} & \textbf{25.61\%} & \textbf{26.36\%} \\ 
    \hline
  \end{tabular}
  \caption{API Call Reduction (\%) by dataset and model.}
  \label{tab:c_api}
\end{table}

\begin{table}[!htb]
  \centering
  \begin{tabular}{|l|l|c|c|c|c|}
    \hline
    {\bfseries Dataset} & {\bfseries Model}   & {\bfseries $P$} & {\bfseries $R$} & {\bfseries $F_1$} & {\bfseries OM-LLM} \\ 
    \hline
    \multirow{4}{*}{Mouse-Human}
      & Debate-2A-3R & 100   & 70    & 82.35 & \multirow{4}{*}{92.20} \\
      & Debate-2A-5R & 100   & 74    & 85.06 &                         \\
      & Debate-4A-3R & 100   & 66    & 79.52 &                         \\
      & Debate-4A-5R & 100   & 68    & 80.95 &                         \\ 
    \hline
    \multirow{4}{*}{Nell-DBpedia}
      & Debate-2A-3R & 97.83 & 90    & 93.75 & \multirow{4}{*}{96}    \\
      & Debate-2A-5R & 95.91 & 94    & 94.95 &                         \\
      & Debate-4A-3R & 95.55 & 86    & 90.53 &                         \\
      & Debate-4A-5R & 93.88 & 92    & 92.93 &                         \\ 
    \hline
    \multirow{4}{*}{YAGO-Wikidata}
      & Debate-2A-3R & 100   & 92    & 95.83 & \multirow{4}{*}{92.19} \\
      & Debate-2A-5R & 100   & 96.88 & 98.41 &                         \\
      & Debate-4A-3R & 100   & 86    & 92.47 &                         \\
      & Debate-4A-5R & 100   & 90    & 94.73 &                         \\ 
    \hline
  \end{tabular}
  \caption{LLM Debate on zero-shot matching performance.}
  \label{tab:d_debate}
\end{table}

\begin{table}[!htb]
  \centering
  \begin{tabular}{|l|l|c|c|c|c|}
    \hline
    {\bfseries Dataset}    & {\bfseries Model}           & {\bfseries $P$} & {\bfseries $R$} & {\bfseries $F_1$} & {\bfseries OM-LLM} \\ 
    \hline
    \multirow{2}{*}{NCIT-DOID}
      & Llama-3.3-70B      & 97.59 & 99.69 & 98.63 & \multirow{2}{*}{94.80} \\
      & DR1D-Llama-3.3-70B & 97.66 & 96.31 & 96.98 &                         \\ 
    \hline
    \multirow{2}{*}{Nell-DBpedia}
      & Llama-3.3-70B      & 94.32 &100.00 & 97.08 & \multirow{2}{*}{96}    \\
      & DR1D-Llama-3.3-70B & 94.67 & 95.48 & 95.07 &                         \\ 
    \hline
    \multirow{2}{*}{YAGO-Wikidata}
      & Llama-3.3-70B      & 91.80 & 99.60 & 95.54 & \multirow{2}{*}{92.19} \\
      & DR1D-Llama-3.3-70B & 92.31 & 94.80 & 93.53 &                         \\ 
    \hline
  \end{tabular}
  \caption{Performance of short vs.\ long reasoning LLMs.}
  \label{tab:e_longshort}
\end{table}

\begin{table}[!htb]
  \centering
  \begin{tabular}{|l|l|c|c|c|}
    \hline
    {\bfseries Dataset}     & {\bfseries Model}           & {\bfseries $P$} & {\bfseries $R$} & {\bfseries $F_1$} \\ 
    \hline
    \multirow{2}{*}{NCIT-DOID}
      & KROMA + Llama-3.1-70B & 97.85 & 98.15 & \textbf{98.00} \\
      & MILA + Llama-3.1-70B  & 96.70 & 92.80 & 94.67      \\ 
    \hline
  \end{tabular}
  \caption{Active learning on NCIT-DOID.}
  \label{tab:f_active}
\end{table}


==> sections/9_discussion.tex <==
\section{Discussion}
